Heterogeneous Multi-task Learning for Human Pose Estimation with Deep Convolutional Neural Network

We propose an heterogeneous multi-task learning framework for human pose estimation from monocular image with deep convolutional neural network. In particular, we simultaneously learn a pose-joint regressor and a sliding-window body-part detector in a deep network architecture. We show that including the body-part detection task helps to regularize the network, directing it to converge to a good solution. We report competitive and state-of-art results on several data sets. We also empirically show that the learned neurons in the middle layer of our network are tuned to localized body parts.

==> img/deep-pose-conv <==
{"contentType":"application/gliffy+json","version":"1.1","stage":{"background":"#FFFFFF","width":1178,"height":587,"nodeIndex":419,"autoFit":true,"exportBorder":false,"gridOn":true,"snapToGrid":true,"drawingGuidesOn":true,"pageBreaksOn":false,"printGridOn":false,"printPaper":"LETTER","printShrinkToFit":false,"printPortrait":true,"maxWidth":5000,"maxHeight":5000,"themeData":null,"objects":[{"x":791.0,"y":289.5550767137935,"rotation":0.0,"id":417,"width":170.4393939393938,"height":48.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":417,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">Full connected layer</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":340.0,"y":540.0,"rotation":0.0,"id":412,"width":85.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":109,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">max pooling</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":220.0,"y":540.0,"rotation":0.0,"id":407,"width":92.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":106,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">convolution</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":1002.0,"y":139.8552997626507,"rotation":0.0,"id":403,"width":180.0,"height":64.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":104,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">classification cost function</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":82.49999999999997,"y":508.0,"rotation":0.0,"id":384,"width":90.0,"height":32.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":91,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">3&#64;112x112</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":870.0,"y":534.0,"rotation":0.0,"id":382,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":90,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":203,"py":1.0,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":251,"py":0.9999999999999998,"px":0.29289321881345254}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-5.0,6.0],[72.86144181197824,-59.745139717266056]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":861.0,"y":361.0,"rotation":0.0,"id":381,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":89,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":203,"py":0.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":251,"py":1.0,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-0.39339828220181516,-1.0],[77.71212121212102,113.25486028273394]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":864.0,"y":539.0,"rotation":0.0,"id":380,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":88,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":203,"py":1.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":251,"py":0.0,"px":0.2928932188134524}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-3.393398282201815,1.0],[78.86144181197824,-135.00337950701044]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":864.0,"y":367.0,"rotation":0.0,"id":379,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":87,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":203,"py":0.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":251,"py":0.0,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-3.393398282201815,-7.0],[74.71212121212102,36.996620492989564]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":848.0,"y":260.0,"rotation":0.0,"id":377,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":86,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":204,"py":0.9999999999999998,"px":0.29289321881345254}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":222,"py":0.5,"px":0.5}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[6.393398282201815,-0.2918642688783848],[86.16666666666663,-90.2918642688783]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":858.0,"y":86.0,"rotation":0.0,"id":376,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":85,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":204,"py":0.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":222,"py":0.5,"px":0.5}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[2.606601717798185,-6.291864268878328],[76.16666666666663,83.7081357311217]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":828.0,"y":540.0,"rotation":0.0,"id":375,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":84,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":200,"py":1.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":203,"py":0.7071067811865475,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-7.393398282201815,0.0],[22.0,-52.72077938642144]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":824.0,"y":363.0,"rotation":0.0,"id":374,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":83,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":200,"py":0.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":203,"py":0.7071067811865475,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-3.393398282201815,-3.0],[26.0,124.27922061357856]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":818.0,"y":538.0,"rotation":0.0,"id":373,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":82,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":200,"py":1.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":203,"py":0.2928932188134525,"px":1.1102230246251563E-16}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[2.606601717798185,2.0],[32.0,-125.27922061357856]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":822.0,"y":365.0,"rotation":0.0,"id":372,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":81,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":200,"py":0.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":203,"py":0.2928932188134525,"px":1.1102230246251563E-16}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-1.3933982822018152,-5.0],[28.0,47.72077938642144]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":832.0,"y":259.0,"rotation":0.0,"id":371,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":80,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":198,"py":1.0,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":204,"py":0.7071067811865475,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-7.0,0.708135731121672],[18.0,-52.01264365529977]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":820.0,"y":84.0,"rotation":0.0,"id":370,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":79,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":198,"py":0.0,"px":0.7071067811865476}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":204,"py":0.7071067811865475,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.6066017177981848,-4.291864268878328],[30.0,122.98735634470023]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":829.0,"y":260.0,"rotation":0.0,"id":369,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":78,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":198,"py":1.0,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":204,"py":0.2928932188134525,"px":1.1102230246251563E-16}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-4.0,-0.29186426887832795],[21.0,-127.57108488245689]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":831.0,"y":86.0,"rotation":0.0,"id":368,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":77,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":198,"py":0.0,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":204,"py":0.2928932188134525,"px":1.1102230246251563E-16}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-6.0,-6.291864268878328],[19.0,46.42891511754311]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":715.0,"y":250.0,"rotation":0.0,"id":366,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":76,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":173,"py":0.5,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":200,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[3.5748108120615143,-3.4952242902413673],[95.0,200.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":734.0,"y":244.0,"rotation":0.0,"id":365,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":75,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":175,"py":0.5,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":200,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[1.5519193886011635,2.5047757097586327],[76.0,206.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":736.0,"y":355.0,"rotation":0.0,"id":364,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":74,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":175,"py":0.5,"px":0.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":200,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-0.4480806113988365,6.100258601401265],[74.0,95.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":718.0,"y":355.0,"rotation":0.0,"id":363,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":73,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":173,"py":0.5,"px":0.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":200,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.5748108120615143,6.100258601401265],[92.0,95.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":712.0,"y":247.0,"rotation":0.0,"id":362,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":72,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":173,"py":0.5,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":198,"py":0.07384369038265738,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[6.574810812061514,-0.49522429024136727],[98.0,-154.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":712.0,"y":359.0,"rotation":0.0,"id":361,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":71,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":173,"py":0.5,"px":0.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":198,"py":0.06828813482710182,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[6.574810812061514,2.100258601401265],[98.0,-267.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":732.0,"y":358.0,"rotation":0.0,"id":360,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":70,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":175,"py":0.5,"px":0.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":198,"py":0.07384369038265738,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[3.5519193886011635,3.100258601401265],[78.0,-265.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":735.0,"y":243.0,"rotation":0.0,"id":359,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":69,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":175,"py":0.5,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":198,"py":0.06273257927154627,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.5519193886011635,3.5047757097586327],[75.0,-152.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":654.0,"y":313.0,"rotation":0.0,"id":356,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":68,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":351,"py":0.5,"px":0.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":173,"py":0.5,"px":0.5}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[1.0,-0.5],[64.57481081206151,-9.197482844420051]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":655.0,"y":285.0,"rotation":0.0,"id":355,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":67,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":351,"py":0.5,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":173,"py":0.5,"px":0.5}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.0,-2.5],[63.574810812061514,18.80251715557995]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":634.0,"y":281.0,"rotation":0.0,"id":353,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":66,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":350,"py":0.5,"px":1.0}},"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":173,"py":0.5,"px":0.5}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[1.0,1.5],[84.57481081206151,22.80251715557995]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":582.0,"y":254.0,"rotation":0.0,"id":339,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":60,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":325,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[3.0,-1.5],[45.0,-12.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":362.0,"y":207.0,"rotation":0.0,"id":298,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":51,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":292,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-4.259854375621671,-3.144700237349298],[90.0,4.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":142.0,"y":280.0,"rotation":0.0,"id":271,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":39,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.0,0.0],[95.0,-10.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":143.0,"y":330.0,"rotation":0.0,"id":270,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":38,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"endConstraint":{"type":"EndPositionConstraint","EndPositionConstraint":{"nodeId":131,"py":0.5,"px":0.5}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.0,0.0],[102.0,-60.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":112.0,"y":322.0,"rotation":0.0,"id":265,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":37,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":263,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-3.6666666666666146,4.666666666666629],[125.0,-53.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":118.0,"y":278.0,"rotation":0.0,"id":264,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":36,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":263,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-9.666666666666629,-9.666666666666686],[119.05223464761411,-9.666666666666686]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":938.712121212121,"y":403.99662049298956,"rotation":0.0,"id":251,"width":14.166666666666742,"height":70.25823978974438,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","order":34,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":110.0,"y":250.0,"rotation":270.0,"id":131,"width":270.0,"height":40.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":6,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":139.0,"y":250.0,"rotation":270.0,"id":132,"width":270.0,"height":40.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":4,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":240.0,"y":450.0,"rotation":0.0,"id":186,"width":68.0,"height":20.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":22,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:12px;font-family:Arial;\"><span style=\"\"><span style=\"font-size:18px;\">...</span><br /></span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":359.8594807238394,"y":416.75486028273394,"rotation":0.0,"id":142,"width":56.666666666666664,"height":20.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":10,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:12px;font-family:Arial;\"><span style=\"\"><span style=\"font-size:18px;\">...</span><br /></span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":242.3594807238395,"y":258.93196492474806,"rotation":270.0,"id":143,"width":224.99999999999997,"height":29.718961447679,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":9,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":463.46449146982917,"y":416.7548602827339,"rotation":0.0,"id":158,"width":50.76561795737565,"height":20.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":13,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:12px;font-family:Arial;\"><span style=\"\"><span style=\"font-size:18px;\">...</span><br /></span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":355.2142767077779,"y":264.779053831121,"rotation":270.0,"id":159,"width":201.5693654189916,"height":31.99791883454735,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":12,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":388.69783292972716,"y":266.75486028273394,"rotation":270.0,"id":161,"width":201.5693654189916,"height":31.99791883454735,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":11,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":639.9445053860798,"y":396.75486028273394,"rotation":0.0,"id":176,"width":37.946643432498185,"height":20.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":18,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:12px;font-family:Arial;\"><span style=\"\"><span style=\"font-size:18px;\">...</span><br /></span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":558.5540535081818,"y":278.0741961439789,"rotation":270.0,"id":177,"width":150.67049598197806,"height":27.77860299834183,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":17,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":583.5825791113398,"y":279.7894684185513,"rotation":270.0,"id":179,"width":150.67049598197806,"height":27.77860299834183,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":0,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":722.8190879561967,"y":383.99662049298956,"rotation":0.0,"id":172,"width":28.86108458011741,"height":20.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":21,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:12px;font-family:Arial;\"><span style=\"\"><span style=\"font-size:18px;\">...</span><br /></span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":661.2770693662402,"y":295.2277063435184,"rotation":270.0,"id":173,"width":114.59548289164263,"height":17.14962162412311,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":20,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":678.2541779427798,"y":295.2277063435184,"rotation":270.0,"id":175,"width":114.59548289164263,"height":17.14962162412311,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":19,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":810.0,"y":360.0,"rotation":0.0,"id":200,"width":15.0,"height":180.0,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","order":24,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":810.0,"y":79.70813573112167,"rotation":0.0,"id":198,"width":15.0,"height":180.0,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","order":23,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":850.0,"y":360.0,"rotation":0.0,"id":203,"width":15.0,"height":180.0,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","order":26,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":850.0,"y":79.70813573112167,"rotation":0.0,"id":204,"width":15.0,"height":180.0,"uid":"com.gliffy.shape.basic.basic_v1.default.rectangle","order":25,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":900.0757575757575,"y":155.54146906445501,"rotation":90.0,"id":222,"width":68.18181818181817,"height":28.333333333333336,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":33,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":904.621212121212,"y":155.54146906445501,"rotation":90.0,"id":221,"width":68.18181818181817,"height":28.333333333333336,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":32,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":909.1666666666665,"y":155.54146906445501,"rotation":90.0,"id":220,"width":68.18181818181817,"height":28.333333333333336,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":31,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":913.7121212121212,"y":155.54146906445501,"rotation":90.0,"id":219,"width":68.18181818181817,"height":28.333333333333336,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":30,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":918.2575757575758,"y":155.54146906445501,"rotation":90.0,"id":218,"width":68.18181818181817,"height":28.333333333333336,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":29,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":922.8030303030303,"y":155.54146906445501,"rotation":90.0,"id":217,"width":68.18181818181817,"height":28.333333333333336,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":28,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":927.3484848484848,"y":155.54146906445501,"rotation":90.0,"id":215,"width":68.18181818181817,"height":28.333333333333336,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":27,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":109.99999999999999,"y":290.0,"rotation":270.0,"id":267,"width":50.0,"height":15.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":3,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":79.16666666666673,"y":290.0,"rotation":270.0,"id":263,"width":58.33333333333329,"height":15.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":35,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":-49.16666666666653,"y":250.0,"rotation":270.0,"id":137,"width":314.9999999999998,"height":40.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":7,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":-37.499999999999886,"y":250.0,"rotation":270.0,"id":6,"width":314.9999999999998,"height":40.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":5,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":-25.83333333333323,"y":250.0,"rotation":270.0,"id":4,"width":314.9999999999998,"height":40.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":2,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":360.22010412223665,"y":257.36952609173824,"rotation":0.0,"id":288,"width":82.66528326194648,"height":100.75312754562684,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":50,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":292,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-2.47995849785832,-3.9150563719196327],[90.9318115881411,-46.346438670988306]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":386.67299476605956,"y":265.42977629538836,"rotation":0.0,"id":289,"width":82.66528326194648,"height":100.75312754562684,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":49,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":291,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[4.133264163097351,-1.8999938210072287],[61.32700523394044,-53.429776295388365]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":389.97960609653745,"y":212.0306186962061,"rotation":0.0,"id":290,"width":82.66528326194648,"height":100.75312754562684,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":48,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":291,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.8266528326194589,1.8999938210071434],[59.520459305263046,-3.526359464096913]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":366.006673950573,"y":231.1737129298752,"rotation":270.0,"id":291,"width":49.599169957167895,"height":15.112969131844027,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":47,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":332.9405606457944,"y":221.09840017531263,"rotation":270.0,"id":292,"width":49.599169957167895,"height":15.112969131844027,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":46,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":242.61633502047488,"y":354.3804717605281,"rotation":0.0,"id":279,"width":96.34604781404686,"height":96.3157337794107,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":45,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":274,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-2.890381434421357,1.4538302170819861],[105.98065259545155,-44.3052375385289]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":273.4470703209699,"y":362.0857304628809,"rotation":0.0,"id":278,"width":96.34604781404686,"height":96.3157337794107,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":44,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":275,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[4.817302390702366,3.3801448926701596],[73.22299633867561,-48.15786688970536]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":277.3009122335318,"y":311.03839155979324,"rotation":0.0,"id":277,"width":96.34604781404686,"height":96.3157337794107,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":43,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":275,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.963460478140405,-3.3801448926702733],[69.37085063831995,-3.3710506822793604]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":240.68941406419395,"y":297.5541888306758,"rotation":0.0,"id":276,"width":96.34604781404686,"height":96.3157337794107,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":42,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":274,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-0.9634604781404335,0.47248445850618737],[109.83449450801339,11.557888053529268]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":249.3605583674582,"y":329.33838097788123,"rotation":270.0,"id":275,"width":57.80762868842811,"height":14.447360066911607,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":41,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":210.82213924183947,"y":319.70680759994025,"rotation":270.0,"id":274,"width":57.80762868842811,"height":14.447360066911607,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":40,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":484.8990646449532,"y":351.1036942538352,"rotation":0.0,"id":304,"width":78.13998539195023,"height":104.40170389714156,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":56,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":307,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[3.90699926959752,-4.2244559151575345],[59.38638889788206,-52.2008519485708]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":275.6928140571728,"y":258.93196492474806,"rotation":270.0,"id":145,"width":224.99999999999997,"height":29.718961447679,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":8,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":459.89426931952914,"y":342.7515579420639,"rotation":0.0,"id":303,"width":78.13998539195023,"height":104.40170389714156,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":57,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":308,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-2.3441995617585007,-6.312489993100257],[85.95398393114522,-48.02478379268507]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":488.02466406063127,"y":295.7707911883502,"rotation":0.0,"id":305,"width":78.13998539195023,"height":104.40170389714156,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":55,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":307,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.7813998539194813,4.224455915157364],[56.262165169116315,-3.654059636399893]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":458.3314696116902,"y":281.1545526427504,"rotation":0.0,"id":306,"width":78.13998539195023,"height":104.40170389714156,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":54,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":308,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-0.7813998539195381,8.40052407104315],[89.07958334682303,12.528204467656963]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":465.3640682969657,"y":315.607114928807,"rotation":270.0,"id":307,"width":46.883991235170136,"height":15.660255584571237,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":53,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":434.1080741401856,"y":305.166944539093,"rotation":270.0,"id":308,"width":46.883991235170136,"height":15.660255584571237,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":52,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":552.4358227598785,"y":396.75486028273394,"rotation":0.0,"id":154,"width":47.56417724012143,"height":20.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":16,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:12px;font-family:Arial;\"><span style=\"\"><span style=\"font-size:18px;\">...</span><br /></span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":454.06765046174144,"y":270.00692553179624,"rotation":270.0,"id":155,"width":188.8577625710704,"height":30.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":15,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":489.9251602752515,"y":270.00692553179505,"rotation":270.0,"id":157,"width":188.8577625710704,"height":30.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":14,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":547.0,"y":222.0,"rotation":0.0,"id":341,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":62,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":338,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[-2.0,0.5],[80.0,19.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":583.0,"y":223.0,"rotation":0.0,"id":340,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":61,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":325,"py":0.5,"px":1.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[2.0,-0.5],[46.0,17.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":540.0,"y":254.0,"rotation":0.0,"id":342,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":63,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":338,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[5.0,-1.5],[84.0,-14.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":530.0,"y":230.0,"rotation":270.0,"id":338,"width":30.0,"height":15.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":59,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":570.0,"y":230.0,"rotation":270.0,"id":325,"width":30.0,"height":15.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":58,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":634.3190879561967,"y":321.9082466671229,"rotation":0.0,"id":349,"width":100.0,"height":100.0,"uid":"com.gliffy.shape.basic.basic_v1.default.line","order":65,"lockAspectRatio":false,"lockShape":false,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":350,"py":0.5,"px":0.0}}},"graphic":{"type":"Line","Line":{"strokeWidth":2.0,"strokeColor":"#000000","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","interpolationType":"linear","cornerRadius":null,"controlPath":[[0.680912043803346,-9.40824666712291],[84.0,-14.0]],"lockSegments":{},"ortho":false}},"linkMap":[],"children":[]},{"x":620.0,"y":290.0,"rotation":270.0,"id":350,"width":30.0,"height":15.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":64,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":640.0,"y":290.0,"rotation":270.0,"id":351,"width":30.0,"height":15.0,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.input_output","order":1,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rhombus.basic_v1","strokeWidth":2.0,"strokeColor":"#333333","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"opacity":1.0,"shadowX":0.0,"shadowY":0.0}},"linkMap":[],"children":[]},{"x":220.0,"y":516.0,"rotation":0.0,"id":387,"width":90.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":92,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">32&#64;104x104</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":339.99999999999994,"y":516.0,"rotation":0.0,"id":388,"width":90.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":93,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">32&#64;52x52</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":440.0,"y":470.0,"rotation":0.0,"id":389,"width":90.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":94,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">16&#64;48x48</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":540.0000000000001,"y":470.0,"rotation":0.0,"id":390,"width":90.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":95,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">16&#64;24x24</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":600.0285256031581,"y":431.1257403878617,"rotation":0.0,"id":391,"width":90.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":96,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">16&#64;20x20</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":679.891148818578,"y":431.1257403878617,"rotation":0.0,"id":392,"width":90.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":97,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">16&#64;10x10</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":837.0,"y":36.5,"rotation":0.0,"id":395,"width":47.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":99,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">512</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":789.0,"y":35.5,"rotation":0.0,"id":393,"width":47.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":98,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">512</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":838.5,"y":571.0,"rotation":0.0,"id":398,"width":47.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":101,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">512</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":790.5,"y":570.0,"rotation":0.0,"id":399,"width":47.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":100,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">512</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":889.1666666666665,"y":79.70813573112167,"rotation":0.0,"id":401,"width":90.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":102,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">7&#64;8x8</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":920.0,"y":500.0,"rotation":0.0,"id":402,"width":47.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":103,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">16</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":1000.0,"y":440.1257403878617,"rotation":0.0,"id":406,"width":180.0,"height":14.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":105,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:12px;font-family:Arial;\"><span style=\"\">regression cost function</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":440.0,"y":492.0,"rotation":0.0,"id":410,"width":92.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":107,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">convolution</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":600.0285256031581,"y":450.0,"rotation":0.0,"id":411,"width":92.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":108,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">convolution</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":541.8540415607869,"y":492.0,"rotation":0.0,"id":415,"width":85.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":110,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">max pooling</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]},{"x":692.0285256031581,"y":450.0,"rotation":0.0,"id":416,"width":85.0,"height":16.0,"uid":"com.gliffy.shape.basic.basic_v1.default.text","order":111,"lockAspectRatio":false,"lockShape":false,"graphic":{"type":"Text","Text":{"overflow":"none","paddingTop":2,"paddingRight":2,"paddingBottom":2,"paddingLeft":2,"type":"fixed","lineTValue":null,"linePerpValue":null,"cardinalityType":null,"html":"<p style=\"text-align:center;\"><span style=\"font-size:14px;font-family:Arial;\"><span style=\"\">max pooling</span></span></p>","tid":null,"valign":"middle","vposition":"none","hposition":"none"}},"linkMap":[],"children":[]}],"shapeStyles":{"com.gliffy.shape.basic.basic_v1.default":{"fill":"#FFFFFF","stroke":"#333333","strokeWidth":2},"com.gliffy.shape.flowchart.flowchart_v1.default":{"fill":"#FFFFFF","stroke":"#333333","strokeWidth":2}},"lineStyles":{"global":{}},"textStyles":{"global":{"size":"14px"}}},"metadata":{"title":"untitled","revision":0,"exportBorder":false,"libraries":["com.gliffy.libraries.basic.basic_v1.default","com.gliffy.libraries.flowchart.flowchart_v1.default","com.gliffy.libraries.swimlanes.swimlanes_v1.default","com.gliffy.libraries.uml.uml_v1.default","com.gliffy.libraries.uml.uml_v2.class","com.gliffy.libraries.uml.uml_v2.sequence","com.gliffy.libraries.uml.uml_v2.activity","com.gliffy.libraries.erd.erd_v1.default","com.gliffy.libraries.ui.ui_v2.forms_components","com.gliffy.libraries.images"]},"embeddedResources":{"index":0,"resources":[]}}
